Cache Where you Want! Reconciling Predictability and Coherent Caching

Real-time and cyber-physical systems need to interact with and respond to their physical environment in a predictable time. While multicore platforms provide incredible computational power and throughput, they also introduce new sources of unpredictability. Large fluctuations in latency to access data shared between multiple cores is an important contributor to the overall execution-time variability. In addition to the temporal unpredictability introduced by caching, parallel applications with data shared across multiple cores also pay additional latency overheads due to data coherence. Analyzing the impact of data coherence on the worst-case execution-time of real-time applications is challenging because only scarce implementation details are revealed by manufacturers. This paper presents application level control for caching data at different levels of the cache hierarchy. The rationale is that by caching data only in shared cache it is possible to bypass private caches. The access latency to data present in caches becomes independent of its coherence state. We discuss the existing architectural support as well as the required hardware and OS modifications to support the proposed cacheability control. We evaluate the system on an architectural simulator. We show that the worst case execution time for a single memory write request is reduced by 52%. Benchmark evaluations show that proposed technique has a minimal impact on average performance.

==> bios.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

% \begin{IEEEbiography}{Michael Shell}
% Biography text here.
% \end{IEEEbiography}

% if you will not have a photo at all:
% \begin{IEEEbiographynophoto}{John Doe}
% Biography text here.
% \end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{Ayoosh Bansal}
is currently a Ph.D. student at University of Illinois at Urbana-Champaign, Dept. of Computer Science.
He received a Bachelors and Masters degree in Electrical Engineering at BITS, Pilani and Univ. of Wisconsin-Madison respectively.
He is a recipient of the Saburo Muroga Endowed Fellowship.
His research interests span over a wide range of topics related to Cyber-Physical Systems and Real-Time Systems, including Safety, Fault Tolerance, Security, Hardware-Software co-design.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Jayati Singh}
received her B. Eng degree from BITS Pilani, India and subsequently joined the Real-Time and Embedded Systems Lab at the University of Illinois at Urbana-Champaign (UIUC). She is currently working as a Researcher at the chair of Cyber-Physical Systems in Production Engineering at TUM under the guidance of Prof. Marco Caccamo. Her research focuses on enhancing the performance of real-time systems at the architecture and OS level.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Yifan Hao}
received his Master of Computer Science degree from University of Illinois at Urbana Champaign. He was supervised by Professor Tarek Abdelzaher and is currently working at VMware. His research interests broadly lie in distributed systems, internet of things and architecture.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Jen-Yang Wen}
is a PhD student in the computer science department at the University of Illinois at Urbana-Champaign. He received his master degree in computer science from the University of Illinois at Urbana Champaign in the year 2019. He received his master degree in electronics engineering from Nation Taiwan University in the year 2010. His main research interests are real-time systems and computer architecture.
\end{IEEEbiographynophoto}

\newpage

\begin{IEEEbiographynophoto}{Renato Mancuso}
is an assistant professor in the Computer
Science Department at Boston University since 2017.
Renato received his Ph.D. from the Department of
Computer Science at the University of Illinois at Urbana-Champaign. 
He is interested in high-performance cyber-physical systems, with a
specific focus on techniques to enforce strong performance isolation
and temporal predictability in multi-core systems. He received a B.S. in
Computer Engineering with honors (2009) and a M.S. in Computer
Engineering with honors (2012) from the University of Rome "Tor
Vergata". He is a member of the IEEE.

\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Marco Caccamo}
studied Computer Engineering at University of Pisa
(Italy). Following his degree in computer engineering in July 1997, he
earned his Ph.D. in computer engineering from Scuola Superiore
Sant’Anna (Italy) in 2002. Shortly after graduation, he joined
University of Illinois at Urbana-Champaign as assistant professor in
Computer Science and was promoted to associate professor at the age of
36, then became a full professor in 2014. Since 2018, Prof. Caccamo
has been appointed to the chair of Cyber-Physical Systems in
Production Engineering at TUM. Caccamo received visiting
professorships at ETH, Zurich and TUM Munich as T\"UV S\"ud Stiftung
visiting professor and August-Wilhelm Scheer guest professor. He has
chaired Real-Time Systems Symposium and Real-Time and Embedded
Technology and Applications Symposium, the two IEEE flagship
conferences on Real-Time Systems. He also served as General Chair of
Cyber Physical Systems Week. In 2003, he was awarded an NSF CAREER
Award. He is a recipient of the Alexander von Humboldt Professorship
and he is IEEE Fellow.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}




